Nuclear Activity and the Conditions of Star-formation at the Galactic Center

The Galactic Center is the closest galactic nucleus that can be studied with unprecedented angular resolution and sensitivity. We summarize recent basic observational results on Sagittarius A* and the conditions for star formation in the central stellar cluster. We cover results from the radio, infrared, and X-ray domain and include results from simulation as well. From (sub-)mm and near-infrared variability and near-infrared polarization data we find that the SgrA* system (supermassive black hole spin, a potential temporary accretion disk and/or outflow) is well ordered in its geometrical orientation and in its emission process that we assume to reflect the accretion process onto the supermassive black hole (SMBH).

==> text.tex <==



Nuclear Activity and the Conditions of
Star-formation at the Galactic Center


A. Eckart, M. Valencia-S., B. Shahzamanian, M. Zajacek, L. Moser, M. Parsa, M. Subroweit, F. Peissker, N. Sabha, M. Horrobin, C. Straubmeier, A. Borkar, D. Kunneriath, V. Karas, C. Rauch, S. Britzen, A. Zensus, M. García-Marín,



11 pages, 4 figures, 1 table

published in PoS-SISSA Proceedings of the: Frontier Research in Astrophysics - II, 23-28 May 2016, Mondello (Palermo), Italy


==> zipit.tex <==


zip 111.zip Eckart_FRAP2016.tex eckart-ALMA.eps eckart-alpha.eps eckart-polorb.eps eckart-spectrum.eps PoS.cls PoSlogo.ps

